Programmable electrical coupling between stochastic magnetic tunnel junctions

Superparamagnetic tunnel junctions (SMTJs) are promising sources of randomness for compact and energy efficient implementations of probabilistic computing techniques. Augmenting an SMTJ with electronic circuits, to convert the random telegraph fluctuations of its resistance state to stochastic digital signals, gives a basic building block known as a probabilistic bit or $p$-bit. Though scalable probabilistic computing methods connecting $p$-bits have been proposed, practical implementations are limited by either minimal tunability or energy inefficient microprocessors-in-the-loop. In this work, we experimentally demonstrate the functionality of a scalable analog unit cell, namely a pair of $p$-bits with programmable electrical coupling. This tunable coupling is implemented with operational amplifier circuits that have a time constant of approximately 1us, which is faster than the mean dwell times of the SMTJs over most of the operating range. Programmability enables flexibility, allowing both positive and negative couplings, as well as coupling devices with widely varying device properties. These tunable coupling circuits can achieve the whole range of correlations from $-1$ to $1$, for both devices with similar timescales, and devices whose time scales vary by an order of magnitude. This range of correlation allows such circuits to be used for scalable implementations of simulated annealing with probabilistic computing.

==> old_appendices.tex <==
\section{\label{sec:Circuit_details}Circuit Details}

This section contains technical details about each amplifier stage in our coupling circuit. There are two inversions on each side of the loop due to the gain stage and the transconductance stage, and an additional inversion can be added to get negative coupling by swapping the op-amp terminals in the threshold stage. All amplifiers are AD820 op-amps.\footnote{{Certain commercial components are identified in this paper to foster understanding. Such identification does not imply recommendation or endorsement by the National Institute of Standards and Technology, nor does it imply that the processes and software identified are necessarily the best available for the purpose.}} In addition to the amplifier stages discussed in the following sections, the circuit also features a slow-turn-on feature and a debugging mode. The slow turn on feature is an RC circuit that slowly applies the desired current to the SMTJ connected to the board to avoid destroying the tunnel barrier. The debugging mode allows us to use a function generator as the input signal on one side of the loop rather than an SMTJ. 

\subsection{Threshold Stage}

\begin{figure}
    \centering
    \includegraphics[width=6.5cm]{figures/threshold_circuit.drawio.pdf}
    \caption{Threshold stage circuit schematic. $I_{fixed}$ is 1~mA and $R_{var}$ is a 1~k$\Omega$ digital potentiometer. This allows us to set the digitization threshold voltage between 0~V and 1~V, which covers the range of switching of our SMTJs.}
    \label{fig:threshold-stage}
\end{figure}

The threshold stage shown in Fig.~\ref{fig:threshold-stage} converts an analog input voltage $V_{in}$ into a digital output voltage $V_{out}$. If $V_{in}$ is above some reference voltage, the output will be high, otherwise it will be low. It consists of an op-amp, a fixed current source, and a variable resistor. The current source and variable resistor together set the digitization reference voltage. The transfer function for the threshold stage is
\begin{equation}
    V_{out} = 
    \begin{cases} 
      0~V & V_{in}\leq I_{fixed}*R_{var} \\
      2.5~V & otherwise\\
   \end{cases}.
\end{equation}
This transfer function is for the positive coupling case, but on our circuit, we have implemented a switch that allows us to change the polarity of the interaction by switching the op-amp inputs. This way, we can have both positive and negative coupling on the same board. 

It should be emphasized that the comparison is done by an op-amp without feedback rather than a digital comparator. Our op-amps are general purpose and have a 1.8~MHz gain-bandwidth product, making them non-ideal for high-speed applications. 

\subsection{Gain Stage}

\begin{figure}
    \centering
    \includegraphics[width=7cm]{figures/gain_stage_circuit.drawio.pdf}
    \caption{Gain stage circuit schematic. $R_1$ is a 100~k$\Omega$ fixed resistor, and $R_{var}$ is a 10~k$\Omega$ digital potentiometer. This makes the gain variable between 0 and 0.1. The output signal is centered at $V_c$ = 1.25~V.}
    \label{fig:gain-stage}
\end{figure}

The gain stage circuit shown in Fig.~\ref{fig:gain-stage} adjusts the voltage difference between high and low levels of the digital output from the threshold stage while keeping it centered at the voltage $V_c$. The voltage difference is proportional to the gain, which is set by $R_{var}$. The transfer function for this stage is
\begin{equation}
    V_{out} = G(V_c - V_{in}) + V_c,
\end{equation}
where $G = R_{var}/R_1$ is the gain. This configuration is inverting: the output changes in the opposite direction as the input.

\subsection{Level Shifting Stage}

\begin{figure}
    \centering
    \includegraphics[width=7cm]{figures/level_shifting_circuit.drawio.pdf}
    \caption{Level shifting stage circuit schematic. In our circuit, $R_1 = R_f = R_2 = R_g = 10~k\Omega$. The output voltage is the input voltage shifted by $V_{bias}$, which is adjusted through digital potentiometers.}
    \label{fig:level-shift-stage}
\end{figure}

The level shifting stage shown in Fig.~\ref{fig:level-shift-stage} takes the scaled gain stage output and shifts the center to a different DC voltage. The transfer function is written as
\begin{equation}
    V_{out} = \frac{(R_1 + R_f)R_g}{(R_2 + R_g)R_1}V_{in} + \frac{(R_1 + R_f)R_2}{(R_2 + R_g)R_1}V_{bias}.
\end{equation}
Taking $R_1 = R_2 = R_g = R_f$, as it is in our circuit, the expression for $V_{out}$ simplifies to
\begin{equation}
    V_{out} = V_{in} + V_{bias}
\end{equation}
This configuration is noninverting. The new center voltage can be adjusted by changing $V_{bias}$. The method for adjusting $V_{bias}$ is similar to the way we set the threshold stage reference voltage in Fig.~\ref{fig:threshold-stage}: with a fixed current source connected to two digital potentiometers of different resolutions. 

% Using the transfer functions from each stage, the change in current levels due to an increment in gain can be determined. \textcolor{red}{derive $\Delta I$ with respect to gain}

\subsection{Transconductance Stage}

\begin{figure}
    \centering
    \includegraphics[width=5cm]{figures/transconductance_circuit.drawio.pdf}
    \caption{Transconductance stage circuit schematic. $V_{dd}$ is 15~V and $R_1$ is 10~$k\Omega$. This circuit converts an input voltage to a proportional output current.}
    \label{fig:transconductance-stage}
\end{figure}

The transconductance stage shown in Fig.~\ref{fig:transconductance-stage} converts the shifted digital signal from the level shifting stage into a proportional current. The transfer function that describes this relationship is 
\begin{equation}
    I_{out} = \frac{V_{dd} - V_{in}}{R_1}
\end{equation}
This configuration is inverting. This output current will be digital, with two discrete levels that move farther apart as $R_{var}$ in the gain stage increases. If this gain stage $R_{var}$ is set to 0~$\Omega$, the difference $2\Delta I$ between discrete current levels is 0~A and the transconductance stage output is a DC current. The adjustable $V_{bias}$ in the level shifting stage allows us to set this DC current. In this way, we can bias the SMTJs to 50~\% or to any point that we choose. The relationship between output current and gain can be derived analytically using these transfer functions.

\appendix

% \section{\label{sec:Circuit_details}Circuit Details}

% This section contains technical details about each amplifier stage in our coupling circuit. There are two inversions on each side of the loop due to the gain stage and the transconductance stage, and an additional inversion can be added to get negative coupling by swapping the op-amp terminals in the threshold stage. All amplifiers are AD820 op-amps.\footnote{{Certain commercial components are identified in this paper to foster understanding. Such identification does not imply recommendation or endorsement by the National Institute of Standards and Technology, nor does it imply that the processes and software identified are necessarily the best available for the purpose.}} In addition to the amplifier stages discussed in the following sections, the circuit also features a slow-turn-on feature and a debugging mode. The slow turn on feature is an RC circuit that slowly applies the desired current to the SMTJ connected to the board to avoid destroying the tunnel barrier. The debugging mode allows us to use a function generator as the input signal on one side of the loop rather than an SMTJ. 

% \subsection{Threshold Stage}

% \begin{figure}
%     \centering
%     \includegraphics[width=6.5cm]{figures/threshold_circuit.drawio.pdf}
%     \caption{Threshold stage circuit schematic. $I_{fixed}$ is 1~mA and $R_{var}$ is a 1~k$\Omega$ digital potentiometer. This allows us to set the digitization threshold voltage between 0~V and 1~V, which covers the range of switching of our SMTJs.}
%     \label{fig:threshold-stage}
% \end{figure}

% The threshold stage shown in Fig.~\ref{fig:threshold-stage} converts an analog input voltage $V_{in}$ into a digital output voltage $V_{out}$. If $V_{in}$ is above some reference voltage, the output will be high, otherwise it will be low. It consists of an op-amp, a fixed current source, and a variable resistor. The current source and variable resistor together set the digitization reference voltage. The transfer function for the threshold stage is
% \begin{equation}
%     V_{out} = 
%     \begin{cases} 
%       0~V & V_{in}\leq I_{fixed}*R_{var} \\
%       2.5~V & otherwise\\
%    \end{cases}.
% \end{equation}
% This transfer function is for the positive coupling case, but on our circuit, we have implemented a switch that allows us to change the polarity of the interaction by switching the op-amp inputs. This way, we can have both positive and negative coupling on the same board. 

% It should be emphasized that the comparison is done by an op-amp without feedback rather than a digital comparator. Our op-amps are general purpose and have a 1.8~MHz gain-bandwidth product, making them non-ideal for high-speed applications. 

% \subsection{Gain Stage}

% \begin{figure}
%     \centering
%     \includegraphics[width=7cm]{figures/gain_stage_circuit.drawio.pdf}
%     \caption{Gain stage circuit schematic. $R_1$ is a 100~k$\Omega$ fixed resistor, and $R_{var}$ is a 10~k$\Omega$ digital potentiometer. This makes the gain variable between 0 and 0.1. The output signal is centered at $V_c$ = 1.25~V.}
%     \label{fig:gain-stage}
% \end{figure}

% The gain stage circuit shown in Fig.~\ref{fig:gain-stage} adjusts the voltage difference between high and low levels of the digital output from the threshold stage while keeping it centered at the voltage $V_c$. The voltage difference is proportional to the gain, which is set by $R_{var}$. The transfer function for this stage is
% \begin{equation}
%     V_{out} = G(V_c - V_{in}) + V_c,
% \end{equation}
% where $G = R_{var}/R_1$ is the gain. This configuration is inverting: the output changes in the opposite direction as the input.

% \subsection{Level Shifting Stage}

% \begin{figure}
%     \centering
%     \includegraphics[width=7cm]{figures/level_shifting_circuit.drawio.pdf}
%     \caption{Level shifting stage circuit schematic. In our circuit, $R_1 = R_f = R_2 = R_g = 10~k\Omega$. The output voltage is the input voltage shifted by $V_{bias}$, which is adjusted through digital potentiometers.}
%     \label{fig:level-shift-stage}
% \end{figure}

% The level shifting stage shown in Fig.~\ref{fig:level-shift-stage} takes the scaled gain stage output and shifts the center to a different DC voltage. The transfer function is written as
% \begin{equation}
%     V_{out} = \frac{(R_1 + R_f)R_g}{(R_2 + R_g)R_1}V_{in} + \frac{(R_1 + R_f)R_2}{(R_2 + R_g)R_1}V_{bias}.
% \end{equation}
% Taking $R_1 = R_2 = R_g = R_f$, as it is in our circuit, the expression for $V_{out}$ simplifies to
% \begin{equation}
%     V_{out} = V_{in} + V_{bias}
% \end{equation}
% This configuration is noninverting. The new center voltage can be adjusted by changing $V_{bias}$. The method for adjusting $V_{bias}$ is similar to the way we set the threshold stage reference voltage in Fig.~\ref{fig:threshold-stage}: with a fixed current source connected to two digital potentiometers of different resolutions. 

% % Using the transfer functions from each stage, the change in current levels due to an increment in gain can be determined. \textcolor{red}{derive $\Delta I$ with respect to gain}

% \subsection{Transconductance Stage}

% \begin{figure}
%     \centering
%     \includegraphics[width=5cm]{figures/transconductance_circuit.drawio.pdf}
%     \caption{Transconductance stage circuit schematic. $V_{dd}$ is 15~V and $R_1$ is 10~$k\Omega$. This circuit converts an input voltage to a proportional output current.}
%     \label{fig:transconductance-stage}
% \end{figure}

% The transconductance stage shown in Fig.~\ref{fig:transconductance-stage} converts the shifted digital signal from the level shifting stage into a proportional current. The transfer function that describes this relationship is 
% \begin{equation}
%     I_{out} = \frac{V_{dd} - V_{in}}{R_1}
% \end{equation}
% This configuration is inverting. This output current will be digital, with two discrete levels that move farther apart as $R_{var}$ in the gain stage increases. If this gain stage $R_{var}$ is set to 0~$\Omega$, the difference $2\Delta I$ between discrete current levels is 0~A and the transconductance stage output is a DC current. The adjustable $V_{bias}$ in the level shifting stage allows us to set this DC current. In this way, we can bias the SMTJs to 50~\% or to any point that we choose. The relationship between output current and gain can be derived analytically using these transfer functions.

% \section{\label{sec:Wobbliness}Device Non-Idealities}

% \begin{figure}
%     \centering
%     \includegraphics[width=8cm]{figures/Wobble_Test.pdf}
%     \caption{(a) Statistical variation in SMTJ AP state probability over 20 trials. (b) Statistical variation in mean dwell time over 20 trials. Each trial is averaged over 10 million points, equivalent to roughly 8000 switches. Trials were done sequentially with a 30 second delay between trials.}
%     \label{fig:wobbly-test}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=8cm]{figures/Noninverting_Identical_Joint_Probability.pdf}
%     \caption{Probability of joint states during positive coupling experiment with SMTJ-1 and SMTJ-2, which have similar switching time scales. The SMTJs used in this work exhibit unstable behavior that causes unreliable statistics. This explains the large variation in probability despite averaging over a sufficient amount of data.}
%     \label{fig:wobbly-probability}
% \end{figure}

% While performing our experiments, we encountered some difficulty setting the SMTJs to a fixed probability of being in either state. Figure~\ref{fig:wobbly-test} displays the results from a test that was conducted to investigate this effect. A fixed current flows through the device, and 10 million points (8000 switches) of data were collected every 30 seconds. The probability calculation is simply the amount of time spent in the AP state divided by the total time. Changing the number of switches had no obvious effect on the probability variation across trials, nor did changing the amount of time between trials. This indicates that the variation is likely to be intrinsic to the devices rather than due to temperature, inaccurate statistics, or other factors related to the experimental setup.

% There are several possible explanations for this variation in probability. One is that our experiments are done without an applied magnetic field, necessitating the use of high currents that are very close to the breakdown current. This can cause fluctuations in the device's resistance. Another is the presence of defects in the SMTJs. It is possible that some parts of the magnetic domain are not switching coherently with the rest of the domain. There is also no temperature control in our setup, so some of the instability we observe could be due to self-heating. 

% The effect of this instability on the coupling experiments is largely unnoticeable in the experimental dwell time plots in Section~\ref{sec:Results} (Fig.~\ref{fig:noninv-identical-corr}(b), Fig.~\ref{fig:inv-identical-corr}(b), and Fig.~\ref{fig:noninv-diff-corr}(b)). However, plotting the probability of each joint state as a function of gain during the coupling experiment, as in Fig.~\ref{fig:wobbly-probability}, clearly shows that this effect impacts our experiments. Using these SMTJs, we are unable to guarantee a fixed probability of being in either state, which is an important aspect of probabilistic computing. Although the SMTJs used in these experiments exhibit some non-ideal behavior, the experimental demonstrations of coupling are no less valid. 

% \section{\label{sec:software}Software routines}
% Several software routines were employed to run the experiment and to increase the accuracy of our results. First, the simulated annealing algorithm includes automatic gain control. The gain is set through a digital potentiometer on the PCB that uses the I2C communication protocol. We use PySerial to send the desired potentiometer update to an Arduino, which then converts the request into an I2C signal for the potentiometer. The second piece of software we developed for this experiment is a closed loop feedback technique for setting the SMTJ to 50~\% probability of being in each state. This is run at the beginning of each experiment so there is no bias towards either state, but if initial bias were desired this technique could easily be used to set the SMTJ to any probability. Due to some unstable behavior observed in our devices, even with this technique it was difficult to set the device to a desired probability. A discussion of this observation can be found Appendix \ref{sec:Wobbliness}. The third software technique we developed is automatic sampling rate adjustment with increasing gain. To get a statistically significant number of switches at high gain, sampling must be done over a much longer period of time, making fast sampling impractical and unnecessary. 

==> old_markov_modeling.tex <==
Since the coupling between SMTJs in our experiments is facilitated entirely by analog circuitry, device properties such as TMR and $I_0$ have less of an impact on the coupling strength or on the behavior of the coupled system than in recent SMTJ coupling work~\cite{talatchian2021mutual,schnitzspan2023electrical}. However, the difference in time scales of the coupled SMTJs does have a sizeable impact on the dynamics of the coupled system. To examine this effect, we can look at the eigenvalues of the Markov transition matrix $\mathbf{M}$ for this system. This is a $4\times 4$ matrix containing the transition rates between each of the four joint states  (P,P), (P,AP), (AP,P),
and (AP,AP), which we index as states 0, 1, 2, and 3, respectively. 

To construct the transition matrix for the coupled system, we refer to Fig.~\ref{fig:markov-tau-plot}(a). This figure provides a conceptual representation of the inverse switching rates of each SMTJ. We consider transitions where both SMTJs switch simultaneously (for instance, a switch from (P,P) to (AP,AP)) to have probability zero; all nonzero transition rates in our system represent single-SMTJ switching events. The switching rate of one SMTJ is dependent on the state of the other SMTJ due to the coupling; in the positive coupling case, when SMTJ-1 is in the P state, the current through SMTJ-2 will be $I_0 - \Delta I$. When SMTJ-1 is in the AP state, the current through SMTJ-2 will be $I_0 + \Delta I$. This tells us which inverse rate in Fig.~\ref{fig:markov-tau-plot}(a) is the correct one for each of the eight possible transitions from one state into another. For example, $1/\tau^+_a$ is the rate for the first SMTJ to switch from the antiparallel state to the parallel state when the second SMTJ is in the antiparallel state and $1/\tau^-_a$ is the rate for the first SMTJ to switch from the parallel state to the antiparallel state when the second SMTJ is in the parallel state. The transition rate diagram is shown in Fig.~\ref{fig:markov-tau-plot}(b).

\begin{figure}
    \centering
    \includegraphics[width=8.5cm]{figures/Markov-transition-diagrams.pdf}
    \caption{(a) Conceptual mean dwell time plot (similar to Fig.~\ref{fig:smtj-characteristics}(b)) showing the inverse switching rates in the two-SMTJ coupled system. Note the log scale on the vertical axis. The mean dwell times in the P and AP states are equal at $I_0$, and these dwell times are labeled as $\tau_{0,1}$ and $\tau_{0,2}$. The remaining labels are dwell times at either $I_0 + \Delta I$ or $I_0 - \Delta I$, which are used to write the transition rates from one state into another. (b) Markov transition diagram for the two-SMTJ coupled system. The switching rate out of each state is effectively a single-device switching rate, which is dependent on the state of the other SMTJ due to coupling.}
    \label{fig:markov-tau-plot}
\end{figure}

Using Eq.~\ref{eq:neel-brown-model}, we have
\begin{align}
    \tau^-\left(I_{0}-\Delta I \right) &=\tau^+\left(I_{0}+\Delta I \right) \\
    \tau^-\left(I_{0}+\Delta I \right) &= \tau^+\left(I_{0}-\Delta I \right).
\end{align}
The notation in Fig.~\ref{fig:markov-tau-plot}(a) can be simplified by taking $\tau_{n}^+ = \tau_{n}^- = \tau_n$, where $n = \{a, b, c, d\}$. Using this simplified notation, the transition rate matrix can be written as
\begin{equation}
    \mathbf{M} = 
    \begin{pmatrix}
        -\frac{1}{\tau_a}-\frac{1}{\tau_c} & \frac{1}{\tau_d} & \frac{1}{\tau_b} & 0 \\[1em]
        \frac{1}{\tau_c} & -\frac{1}{\tau_b}-\frac{1}{\tau_d} & 0 & \frac{1}{\tau_a} \\[1em]
        \frac{1}{\tau_a} & 0 & -\frac{1}{\tau_b}-\frac{1}{\tau_d} & \frac{1}{\tau_c} \\[1em]
        0 & \frac{1}{\tau_b} & \frac{1}{\tau_d} & -\frac{1}{\tau_a}-\frac{1}{\tau_c}
    \end{pmatrix}, \nonumber
\end{equation}
where $M_{ij}$ is the transition rate departing from state $j$ and arriving in state $i$. The columns of $\mathbf{M}$ sum to $0$, as required by conservation of probability.

At present, the entries of $\mathbf{M}$ are generic time scales. To make $\mathbf{M}$ more concrete, we can use Eq.~\ref{eq:neel-brown-model} to express these $\tau$s in terms of their respective $\tau_{0}$s as
\begin{align}
    \tau^+(I_{0}) = \tau^-(I_{0}) &= \tau_{0} = A \nonumber \\
    \tau^+\left(I_{0}+\Delta I \right) &= Ae^{B\Delta I} \label{eq:tau_one}\\
    \tau^+\left(I_{0}-\Delta I \right) &= Ae^{-B\Delta I}, \label{eq:tau_two}
\end{align}
defining $A = \tau_{att} \exp\left[{\Delta E}/{kT}\right]$ and $B = {\Delta E}/{kTI_c}$. We can represent the difference in time scales by a scaling factor $r$ on $\tau_{0}$ via
\begin{equation}
    \tau_{0,1} = r\tau_{0,2}.
\end{equation}
We can let $g = \exp\left[B\Delta I\right]$ represent the change in the dwell times as a function of gain ($G$), since $\Delta I$ is linearly related to the gain. For the sake of clarity, we have chosen to make $g$ for the two SMTJs equal. This implies that $B$ for the two SMTJs are equal, which would make the slopes of the lines in Fig.~\ref{fig:markov-tau-plot}(a) equal. We can then rewrite each of the $\tau_n$s in Fig.~\ref{fig:markov-tau-plot}(a) by substituting $g$ and the $\tau_0$s into Eqs.~\ref{eq:tau_one} and \ref{eq:tau_two}. The new $\tau_n$s are
\begin{equation}
    \begin{split}
        \tau_{a} &= g\tau_{0,1} \nonumber\\
        \tau_{b} &= \frac{1}{g}\tau_{0,1} \nonumber
    \end{split}
    \quad\quad\quad
    \begin{split}
        \tau_{c} &= \frac{g}{r}\tau_{0,1} \nonumber\\
        \tau_{d} &= \frac{1}{gr}\tau_{0,1}. \nonumber
    \end{split}
\end{equation}
Note that although the gain $G$ is proportional to the current increment $\Delta I$ , $g$ is an exponential function of both $G$ and $\Delta I$. 

Substituting these $\tau_n$s in the transition matrix; the resulting matrix is
\begin{equation}
    \mathbf{M} = \frac{1}{\tau_{0,1}}
    \begin{pmatrix}
        -\frac{1}{g}-\frac{r}{g} & gr & g & 0 \\[1em]
        \frac{r}{g} & -g-gr & 0 & \frac{1}{g} \\[1em]
        \frac{1}{g} & 0 & -g-gr & \frac{r}{g} \\[1em]
        0 & g & gr & -\frac{1}{g}-\frac{r}{g}
    \end{pmatrix}.\nonumber
\end{equation}

The probability distribution describing the system evolves according to the master equation $d\mathbf{P}(t) = \mathbf{M}\mathbf{P}(t)\,dt$, which has the general solution
\begin{equation}
    \mathbf{P}(t) = \exp(\mathbf{M}t)\mathbf{P}_0.
\end{equation}

Following the discussion in Appendix B of Ref.~\cite{talatchian2021mutual}, $\mathbf{P}(t)$ can be expressed as a linear combination of the eigenvalue ($e^{\lambda_{i}t}$) terms multiplied with the time-independent eigenvectors. Since $\mathbf{M}$ is a singular matrix, it has one eigenvalue equal to zero; the other three eigenvalues are negative. Thus, there will be one eigenvector that does not decay, namely the steady state probability distribution. The eigenvector corresponding to the zero eigenvalue in our $\mathbf{M}$ matrix is 
\begin{equation}
    v_0 = \left(1, \frac{1}{g^2}, \frac{1}{g^2}, 1 \right).
\end{equation}
Note that this eigenvector, which encodes the (unnormalized) steady state distribution, is only a function of $g$, and the probability of being in the two disfavored states decreases quadratically with the value of $g$. Note that $g$ itself depends exponentially on the gain.

In addition to this zero eigenvalue, there are three negative eigenvalues. The largest of these (the one closest to positive infinity) provides the slowest rate of decay into the steady state distribution. In order to see how selecting SMTJs with different time scales affects the coupled dynamics, we can look at the eigenvalue that produces the term which decays most slowly,
\begin{gather}
    \lambda_1 = \frac{1}{\tau_{0,1}}  \frac{-b+\sqrt{-16g^2r+b^2}}{2g} \\
    b = (g^2+1)(r+1), \nonumber
\end{gather}
which depends on both $g$ and $r$. So although the final distribution is governed by $g$ alone, the time scale of the coupled system's relaxation to equilibrium increases not only with gain but also with a higher ratio of SMTJ time scales. 

We use this model to predict the mean joint dwell times during the coupled experiments. These model predictions are plotted as solid lines on the experimental dwell time plots in Section~\ref{sec:Results} (Fig.~\ref{fig:noninv-identical-corr}(b), Fig.~\ref{fig:inv-identical-corr}(b), and Fig.~\ref{fig:noninv-diff-corr}(b)). To apply the model to our experiment, we drop the assumption that $B$ is the same for both SMTJs. This is not true in our case. The result of this is that each SMTJ has its own $g$ value, and the steady state distribution becomes dependent on $r$ in addition to $g$. We fit lines to the characteristic dwell time plots of Fig.~\ref{fig:smtj-characteristics} to obtain $B$, which we use to calculate $g$ for each SMTJ. $\tau_{0,1}$ and $r$ were also determined from Fig.~\ref{fig:smtj-characteristics} for each pair of SMTJs. The negative reciprocals of the diagonal elements of $\mathbf{M}$ give the dwell times in each of the four joint states for a given $\Delta I$. 

==> oldpaperandfigs.tex <==
% Magnetic tunnel junctions (MTJs) are nanoscale magnetic devices that consist of two ferromagnetic layers separated by a thin insulator~\cite{jinnai2020scaling}. The insulating layer is thin enough for electrons to tunnel from one ferromagnetic layer to another. The resistance seen by the tunneling electrons depends on the relative orientation of the magnetizations of the ferromagnetic layers~\cite{julliere1975tunneling}. There are two stable configurations of the magnetizations, namely parallel and antiparallel (denoted as P and AP). The device resistance, also known as the tunnel magnetoresistance (TMR), is smaller if the magnetizations are parallel to each other than if they are antiparallel~\cite{moodera1995large}. The relative orientations between layers can be changed by applying an external magnetic field across the device or passing a current through the device~\cite{slonczewski1996current,ralph2008spin}.% through an effect called spin-transfer torque. 

% MTJs have various properties that make them useful as memory devices when integrated into modern complementary metal oxide semiconductor (CMOS) chips~\cite{worledge2022spin,garello2019manufacturable}. Their stable configurations are used to encode binary values: for example, the parallel state may encode a value of \textbf{0} and the antiparallel state a value of \textbf{1}. When used in storage applications~\cite{lee20191gbit,aggarwal2019demonstration} requiring long retention times ($\approx 10$ years), the energy barrier between stable configurations is engineered to be $\geq 40~kT$, where $k$ is Boltzmann's constant and $T=300$~K is room temperature. Sensing the device resistance can be accomplished with a small read voltage (tens of millivolts) that does not disturb the device state, allowing high read endurance~\cite{yuasa2004giant}. As larger voltages are applied across the device, spin polarized tunneling currents apply a spin transfer torque~\cite{stiles2002anatomy,li2003magnetization} on one of the layers. This causes its magnetization to flip, writing the device to a different state. The current-controlled tunability of resistance, non-volatility, back-end-of-the-line (BEOL) CMOS compatibility~\cite{aggarwal2019demonstration}, and aggressive lithographic scalability ($\leq 100$~nm) make MTJ-based magnetic random access memory (MRAM) a promising candidate for various memory and unconventional computing applications~\cite{grollierNeuromorphicSpintronics2020,aggarwal2019demonstration,jung2022crossbar,dong20181,golonzka2018mram}.

% Reducing the energy barrier reduces exponentially the retention time of the MTJ~\cite{kanai2021theory,rippard2011thermal}. For energy barriers less than $14~kT$, thermal fluctuations at room temperature  switch the device between its stable configurations~\cite{bapna2017current} at time scales faster than a millisecond. In this regime, devices are said to be superparamagnetic. A current applied across the device allows its fluctuating resistance state to be read out as a random telegraph voltage signal and simultaneously controls the relative time that the device spends in each of its stable states~\cite{rippard2011thermal}. The ability to generate tunable random signals makes superparamagnetic tunnel junctions (SMTJs) useful for applications where cheap, energy-efficient randomness is required~\cite{daniels2020energy,shukla2023,schnitzspan2023nanosecond,vodenicarevic2017low}. Conventional CMOS sources of randomness such as linear feedback shift registers are only pseudo-random and require comparatively large area and energy budgets~\cite{daniels2020energy}. 

% One promising use for SMTJs is in probabilistic computing. The central objects in probabilistic computers are probabilistic bits, also known as $p$-bits~\cite{camsari2017stochastic}. Unlike a conventional Boolean bit, which takes only deterministic \textbf{1} and \textbf{0} values, a $p$-bit uses its room-temperature instability to encode a probability value. This is particularly useful in applications such as energy-based machine learning models~\cite{kaiser2022hardware,aadit2021computing}, combinatorial optimization~\cite{aadit2022massively}, and quantum simulation~\cite{lucas2014ising,chowdhury2023accelerated}.

% These applications map their problem statements into graphs of interconnected binary nodes with variable interaction strengths~\cite{aadit2022massively}. The parameters of the problem at hand are encoded in the interaction strengths, while the collective configuration of the binary nodes encodes the current proposed solution. The interaction strengths define an effective energy for each global configuration~\cite{pervaiz2018weighted}. If the state of each node is probabilistic, the configuration evolves with time and can explore configuration space according to a Boltzmann distribution, tending to spend more time in configurations with lower effective energy. In an algorithm referred to as simulated annealing~\cite{bertsimas1993simulated}, the interaction strengths can be collectively increased in a way analogous to lowering the temperature so that the configuration spends more time in the lowest energy state until a solution within the required error margin is achieved. 

% Implementing such calculations on conventional computing systems can be time-consuming and inefficient. For large problems, the interconnection weights are necessarily stored on off-chip memory, while iterative calculations of the solution are performed on chip~\cite{jouppi2017datacenter}. Since conventional computing systems have separate locations for memory and computation most of the performance limitations arise from having to move data between memory and computation centers~\cite{wulf1995hitting} (the so-called von Neumann bottleneck). SMTJ-based $p$-bit networks can help alleviate some of these concerns. Using stochastically fluctuating $p$-bits as the nodes, a large binary state space can be efficiently searched in both area and energy cost. Moreover, their density allows them to be packed into large arrays with locally engineered, electronically tunable interactions between them. This allows memory (interaction strengths) and computation (accumulation and randomness generation) to be co-located, promising significant performance boosts~\cite{sebastian2020memory}. 

% Though many proposals of large-scale probabilistic computing systems using $p$-bits have been reported in literature \cite{aadit2022massively,chowdhury2023accelerated,borders2019integer}, practical implementations are still limited to a handful of devices. The largest demonstrations use up to 80 $p$-bits and perform tasks such as integer factorization~\cite{borders2019integer}, invertible logic gates~\cite{camsari2017stochastic}, and learning Boolean functions~\cite{kaiser2022hardware} and travelling salesman problems~\cite{si2023energy}. Larger scale demonstrations are limited by practical factors such as a lack of integrated platforms for exploration, yield and repeatability failures in the fabrication process, the need for an external magnetic field, and differences in time scales between memory and computation. External magnetic fields in particular, which are required to set devices in the superparamagnetic regime in many experiments, are inefficient and impractical in commercial applications. 

% Mismatch of timescales is an especially important issue. A key requirement for correct operation of probabilistic circuits is that the computation necessary to determine the next state in configuration space must complete before the states flip thermally. In other words, the time scales of the interaction circuits (which can become relatively complex), must be smaller than the timescales of nodes themselves. Previous demonstrations~\cite{borders2019integer,kaiser2022hardware,si2023energy} measure the device state and perform the calculations of the accumulated interactions with a microprocessor in the loop. This is only possible because the devices have switching times in the tens of milliseconds or more, which is enough for thousands of microprocessor cycles to perform computations digitally. 

% Though using a microprocessor in the loop is useful to demonstrate the functionality and expressibility of probabilistic computing, it is impractical for scalable implementations. Yet recent papers report simple ways of directly coupling devices. When two SMTJs are connected in parallel~\cite{talatchian2021mutual,phan2022electrical} or in series~\cite{mizrahi2016synchronization,schnitzspan2023electrical} to a voltage source via a tunable resistor, the current flowing through one device depends on the state of the other. Though such approaches can scale theoretically~\cite{daniels2023neural}, practical problems such as line resistance, device-to-device variability, and noise quickly overwhelm linear circuit solutions as the number of devices grows. %While such approaches can correlate devices they do not provide the flexibility to implement arbitrary interactions when scaled up to many devices.  

% The fastest and most energy-efficient implementations would consist of CMOS integrated with SMTJs in the back end of the line~\cite{jung2022crossbar}. Such implementations would involve analog stages mediating interactions between SMTJ-based $p$-bit unit cells. In this work, we take a step in that direction with commercial off-the-shelf (COTS) analog circuits. We experimentally demonstrate the functionality of a unit cell coupling circuit between $p$-bits, with direct analog interaction between field-free SMTJs that have operational time scales in the tens to hundreds of microseconds. The speeds of the analog computation circuits themselves are much faster, on the order of 1~{\textmu}s, allowing the devices to faithfully couple to each other. The degree of coupling can be tuned by varying the interaction strengths, while the uncoupled probabilities of the devices can be independently set by adjusting bias currents. These two features, coupled with a programmable gain circuit, provide the necessary ingredients to perform optimization based on simulated annealing. This unit cell can be readily adapted to couple more than two devices, making it a useful stepping stone towards integration of arrays of devices. 
% %\textcolor{red}{reflect that the COTS prototype is going to be similar to what will be designed for integrated systems }

% The rest of the paper is organized as follows. Section~\ref{sec:circuit} describes the details of the various stages of the coupling circuits and their functionality. Section~\ref{sec:engineering} discusses the experimental setup and the details of the specific SMTJs used. Section~\ref{sec:Results} describes the experimental results of coupling devices of various time scales, and Sec.~\ref{sec:MarkovModelling} describes a Markov model that accurately describes the switching time scales of the two-SMTJ coupled system.

% \begin{figure}
%     \centering
%     \includegraphics[width=7cm]{figures/Simple_Coupling_Block_Diagram.pdf}
%     \caption{Conceptual representation of SMTJ coupling circuit. Each SMTJ can be biased through $I_{bias}$  to a specific initial set of probabilities in the absence of interaction, which is then tuned by setting the gain $G$, which multiplies a preset current increment, $\Delta I$. $V_{mid}$ is the threshold for digitization, ideally halfway between the P and AP state voltage levels. This pairwise interaction circuit could be used as a unit cell in an Ising machine, where the exchange interaction between spins is tuned via the gain.}
%     \label{fig:ising-unit-cell}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=8.5cm]{figures/Circuit_Stage_Outputs.pdf}
%     \caption{ Block diagram representation of interaction circuit. This figure is an expansion of the tunable interaction block in Fig.~\ref{fig:ising-unit-cell}. The SMTJ voltage gets sensed by a threshold stage, with $V_{mid}$ as the programmable threshold. This stage converts the stochastic fluctuations to a digital signal. This digital signal is passed through a gain stage, which adjusts the magnitude of this digital signal while retaining the mid voltage level. The gain ($G$) is programmable. The level shifting stage adjusts the mid voltage level while retaining the voltage difference between high and low levels. $V_{bias}$ controls the size of the shift. Finally, the shifted voltage is converted to a fluctuating current, which facilitates the interaction between SMTJs. In this example, the output current is an inverted version of the SMTJ state, but both positive and negative coupling are possible with our circuit In this example, $V_{mid} = 615~mV$, $G = 0.05$, and $V_{bias} = 5.5~V$.}
%     \label{fig:circuit-output-stages}
% \end{figure}

%When the CoFeB free layer within the magnetic stack is finely adjusted to a thickness of approximately 1.4~nm, the resulting decrease in interfacial perpendicular magnetic anisotropy becomes significant enough to nearly compensate the self-demagnetization field caused by the cylindrical geometry of the free layer. As this near balance is approached, the energy barrier separating the stable perpendicular orientations reduces considerably. This reduction leads to stochastic magnetization fluctuations, indicative of a superparamagnetic regime.

% We use two metrics to quantify the strength of the coupling: Pearson correlation and mean joint dwell times. Both of these metrics can be extracted from the switching data of the coupled SMTJs. We define as joint states the four microstates of the two-SMTJ system: (P,P), (P,AP), (AP,P), and (AP,AP). We define joint dwell times to be the mean dwell times in each of these four joint states. Coupling can be further observed in the bivariate histograms of SMTJ voltages, which quantify the probability density of voltage pairs. The joint state probability mass distributions are coarse-grainings of these analog voltage histograms.

% The Pearson correlation between the voltage-time traces of the the two SMTJs highlights the coupling when the coefficient is plotted as a function of gain. This is plotted in Fig.~\ref{fig:noninv-identical-corr}(a) for positive coupling between two SMTJs of similar time scales (SMTJ-1 and SMTJ-2 in Fig.~\ref{fig:smtj-characteristics}). The increase in the correlation coefficient between the two SMTJ voltage-time traces with gain demonstrates that the SMTJs are have a larger impact on each other's behavior in that regime. Previous demonstrations of coupling between SMTJs \cite{talatchian2021mutual,phan2022electrical,schnitzspan2023electrical} yielded a maximum Pearson correlation coefficient of $0.35$, while ours approaches $1$.

% Plotting the mean dwell times of the joint states also demonstrates coupling of the SMTJs, as seen in Fig.~\ref{fig:noninv-identical-corr}(b). Due to positive coupling, the SMTJs influence each other to be in the same state, so they spend more time in the joint states (P,P) and (AP,AP) and less time in the joint states (P,AP) and (AP,P) as the gain increases. 

% Note that the (P,AP) and (AP,P) dwell times decrease linearly until around $G = 0.03$, where the curve begins to flatten out. This is a sampling artifact. As the gain increases, the sampling rate is automatically decreased to sample for longer times without collecting more points. Once the time scales differ too widely, it becomes prohibitive to collect enough data for good statistics on the large dwell times without missing some of the short dwell time events. For this reason, we truncate the current range over which we compute dwell times. This mismatch in time scales will not be as significant for simulating annealing because probabilities converge more quickly than dwell time distributions.

% The log-scale bivariate histograms of Fig.~\ref{fig:noninv-identical-energy} provide a more dynamic representation of the system's behavior. These plots span the voltages across SMTJ-1 and SMTJ-2, dividing each voltage axis into $100$ bins, and counting the number of points that fall into each 2-dimensional voltage-state bin.  These histograms indicate a high density of occurrence in the (P,P) and (AP,AP) states at high gain, with less time spent in the (P,AP) and (AP,P) states. Note the banded pattern that emerges in these histograms with increasing gain. When one SMTJ initiates a switch out of the (P,P) or (AP,AP) states, it takes approximately 1~{\textmu}s for the current through the other SMTJ to update. Only once the update takes place does the voltage increases accordingly, causing two discrete voltage levels to appear in the histogram. %Switches out of these pseudo-states create the banded pattern.

% Using the same two SMTJs with similar time scales (SMTJ-1 and SMTJ-2 in Fig.~\ref{fig:smtj-characteristics}), we repeated the experiment using negative coupling. Fig.~\ref{fig:inv-identical-corr}(a) shows the Pearson correlation coefficient for this negative coupling experiment. In this case, the SMTJs influence each other to be in opposite states. We observe a strong anticorrelation that approaches $-1$ at $G = 0.06$. Fig.~\ref{fig:inv-identical-corr}(b) shows the mean joint dwell times for the negative coupling experiment. Here the SMTJs spend more time in the antisymmetric joint states (P,AP) and (AP,P) -- and less time in the symmetric joint states (P,P) and (AP,AP) -- as the gain increases. 

% We then repeated the experiment a third time to demonstrate positive coupling between two SMTJs with different time scales (SMTJ-2 and SMTJ-3 in Fig.~\ref{fig:smtj-characteristics}). The plot of Pearson correlation coefficient in Fig.~\ref{fig:noninv-diff-corr}(a) demonstrates a maximum correlation approaching $1$, and the mean joint dwell time plot of Fig.~\ref{fig:noninv-diff-corr}(b) shows that the SMTJs spend more time in the symmetric joint states (P,P) and (AP,AP) and less time in the antisymmetric joint states (P,AP) and (AP,P) as the gain increases. The histograms in Fig.~\ref{fig:noninv-diff-energy} clearly exhibit the effect of differing time scales on the behavior of the system. The faster SMTJ (on the vertical axis) creates a higher density of points between vertical levels due to the higher number of switching attempts compared to the slower SMTJ on the horizontal axis.



\begin{figure}
    \centering
    \includegraphics[width=8.5cm]{figures/Noninverting_Different_Energy.pdf}
    \caption{Bivariate histogram of SMTJ voltages during positive coupling experiment with SMTJ-2 and SMTJ-3. Since SMTJ-3 has shorter dwell times than SMTJ-2, it spends a higher fraction of its time in the transitions and hence is more likely to be sampled there, leading to a higher density of points between states. At $0.06$ gain, SMTJ-3 tends to initiate switches out of joint states (P,P) and (AP,AP), but it also tends to switch back before SMTJ-2 responds to   the change in current. The banded pattern that emerges as the (P,AP) and (AP,P) states become less probable is due to the propagation delay in our circuit.}
    \label{fig:noninv-diff-energy}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=8.5cm]{figures/Noninverting_Identical_Energy.pdf}
    \caption{Bivariate histogram of SMTJ voltages during positive coupling experiment with SMTJ-1 and SMTJ-2. In the zero gain case, the four joint states have roughly equal probability. As the gain increases, the density of points in the two joint states (P,AP) and (AP,P) decreases and a banded pattern begins emerging. This banding is a result of the propagation delay in our circuit.}
    \label{fig:noninv-identical-energy}
\end{figure}

%The dynamics of the interaction can be observed in the log-scale bivariate histograms of SMTJ voltages in Fig.~\ref{fig:noninv-identical-energy}, which quantify the probability density of voltage pairs at different values of gain. The joint state probability mass distributions are coarse-grainings of these analog voltage histograms. These plots span the voltages across SMTJ-1 and SMTJ-2, dividing each voltage axis into $100$ bins, and counting the number of points that fall into each 2-dimensional voltage-state bin. These histograms indicate a high density of occurrence in the (P,P) and (AP,AP) states at high gain, with less time spent in the (P,AP) and (AP,P) states. Note the banded pattern that emerges with increasing gain. When one SMTJ initiates a switch out of the (P,P) or (AP,AP) states, it takes approximately 1~{\textmu}s for the current through the other SMTJ to update. Only once the update takes place does the voltage increase accordingly, causing two discrete voltage levels to appear in the histogram. 

%The main difference between the similar and differing time scale experiments is seen in the histograms of Fig.~\ref{fig:noninv-diff-energy}. The faster SMTJ (on the vertical axis) creates a higher density of points between vertical levels due to the higher number of switching attempts compared to the slower SMTJ on the horizontal axis
